Who Would be Interested in Services? An Entity Graph Learning System for User Targeting

With the growing popularity of various mobile devices, user targeting has received a growing amount of attention, which aims at effectively and efficiently locating target users that are interested in specific services. Most pioneering works for user targeting tasks commonly perform similarity-based expansion with a few active users as seeds, suffering from the following major issues: the unavailability of seed users for newcoming services and the unfriendliness of black-box procedures towards marketers. In this paper, we design an Entity Graph Learning (EGL) system to provide explainable user targeting ability meanwhile applicable to addressing the cold-start issue. EGL System follows the hybrid online-offline architecture to satisfy the requirements of scalability and timeliness. Specifically, in the offline stage, the system focuses on the heavyweight entity graph construction and user entity preference learning, in which we propose a Three-stage Relation Mining Procedure (TRMP), breaking loose from the expensive seed users. At the online stage, the system offers the ability of user targeting in real-time based on the entity graph from the offline stage. Since the user targeting process is based on graph reasoning, the whole process is transparent and operation-friendly to marketers. Finally, extensive offline experiments and online A/B testing demonstrate the superior performance of the proposed EGL System.

==> sec-preliminaries.tex <==

\section{Preliminaries}
In this section, we first briefly introduce the architecture
of the proposed framework of TSEEMP. Then we review the basics of
knowledge, based on which the modules in our model will be
developed. Our proposed architecture consists of three stages: Candidate Generation Stage, Ranking Stage, Ensemble Stage. 


The stage of candidate generation is based on both a Skip-gram model
where the objective function is extended by leveraging word pairs constructed using the descriptions of entities and a bert model. The ranking stage mainly use link prediction model based on graph neural networks. Now we introduce the mentioned preliminaries for our methodologies in sequence.

\subsection{Bert}
BERT is a pre-trained model proposed by Google AI Research Institute in October 2018. BERT is Bidirectional Encoder Representation from Transformers. BERT has shown amazing results with SQuAD1.1, the top level machine reading comprehension test: MultiNLI is highly expressed in 11 different NLP tests. The SOTA performance was achieved by increasing the GLUE benchmark to 80.4\% (7.6\% absolute improvement) and MultiNLI accuracy to 86.7\% (5.6\% absolute improvement). This is a landmark model achievement in the history of NLP. In our scenario, we use bert to generate the initial edge between entities.

\subsection{Skip-gram}
Word embedding has been demonstrated to be an effective
tool in capturing semantic relationships of the words.
Represented by dense vectors, words with similar semantic
and syntatic attributes can be found in the same area in the
continuous vector space. One of the most successful word
embedding methods is proposed by Mikolov \cite{mikolov2013efficient}, known as Skip-Gram with Negative-Sampling (SGNS). The objective
function of SGNS is expressed as:
\begin{equation}\label{eqn-1} 
  log \sigmoid(w*c) + k* E_{c_{neg}~p(c)}[log \ \sigmoid(-w*c_{neg})]
\end{equation}

where w and c represent word and one of its contexts in a
sliding window, respectively. $w \in R^K and c \in RK$ are vector
representations of them. $\sigmoid(w*c)= 1/ (1 + e^{−w·c}).$ $c_{neg}$ is
the sampled contexts, known as negative samples, drawn based
on a unigram distribution $p(c)$. k is the number of negative
samples.


\subsection{Link Prediction}
Link prediction is to predict that whether two nodes in a network are likely to have a link.Consider a network $G=(V,E)$, where $V$ represents the entity nodes in the network and $E \in |V| \times |V|$ represents the set of true links across entities in the network. We are given the set of entities $V$ and a subset of true links which are referred to as observed links. The goal of link prediction is to identify the unobserved true links. Our scene falls into the binary classification formulation of the link prediction task, in which the potential links are classified as either true links or false links. 
In this setting we need to learn a classifier ${M_{b}}$ that maps links in $E'$ to positive and negative labels i.e. ${\displaystyle M_{b}:E'\to \{0,1\}}$.

\subsection{Graph Neural Networks}
Recently, graph neural networks (GNNs) have
advanced the representation learning of vertices atop of underlying
graphs in irregular domains, and help the applications
ranging from social networks \cite{2017Inductive}, transaction networks \cite{2018Heterogeneous}, and gene expression networks \cite{2018Protein}. A GNN usually consists of graph convolution layers which extract local substructure features for individual nodes, and a graph aggregation layer which aggregates node-level features into a graph-level feature vector. Given the ubiquitous existence of networks recently, GNN based link prediction performs
relatively good in many scenarios (\cite{zhang2018link}). Hence we will use GNN as basic component of our link prediction model.

%\subsection{Ensemble}



==> sec-rel.tex <==
\section{Related Works}
\subsection{Potential user clustering}
Methods of potential user clustering mainly can be categorized into two lines:
rule-based and look alike based methods.
The rule-based methods \cite{mangalampalli2011feature,shen2015effective} match potential users of the service with specific demographic tags (age, gender, geography) or interests that are targeted by marketers. The core technical support in the background is user profile mining, which means that the interest tags are inferred from the user behaviour. However, these methods only capture the high-level feature, which is hard to achieve satisfying performance. The look-alike model based methods expand a given seed set via calculating the similarity of all pairs between seed users
and candidate users \cite{ma2016score,liu2016audience} or training customized prediction models for each service or campaign \cite{zhuang2020hubble,zhu2021learning}. These methods show good performance in potential user clustering of services but need seed users. Hence both of the methods cannot solve the problems we face.
% Qu et al. [23] utilized LR to expand audiences, which is effective. In
% terms of audience expansion performance, [7] studied the impact of
% sampling ratios and sampling techniques. These one-stage methods
% train customized models from scratch for each campaign which is
% time-consuming and suffers from the overfitting problem. Recently,
% some two-stage approaches [2, 13, 35] have been proposed to pretrain
% the embedding with data of all campaigns. However, these


\subsection{Link prediction}

Previous work for link prediction can be divided into the heuristic methods, network embedding, and supervised methods. Heuristic methods usually assume that nodes with links satisfy some specific properties. For instance, common neighbor \cite{liben2007link} defines the similarity as the number of shared neighbors of two nodes. Jaccard Coefficient [33] is similar to the common neighbor but normalizes the above score,
as given below.
Katz index \cite{katz1953new} calculates similarity by counting the number of reachable paths. These heuristic methods rely on hand-crafted rules and have strong assumptions, which can not be applied to all kinds of networks. Recently, a number of researchers propose to perform link prediction through constructing node latent features, which are learned via classical matrix factorization \cite{shi2018heterogeneous} and shallow graph representation learning (e.g., Deepwalk \cite{perozzi2014deepwalk} ,Line \cite{tang2015line}, Node2Vec \cite{grover2016node2vec}). And there is also research \cite{zhang2018link,teru2020inductive} inductively predicts node relations by leveraging graph neural networks, which combine high-order topological and initial features in the form of graph patterns. The supervised models  have significantly advanced the state of the art in the past few years. However, these approaches are hard to explicitly provide a personalized decision boundary for a certain source node to determine if other nodes are related to the source node. And there are not any studies about the sample selection problems of link prediction task.

%\subsection{Entity Graph}



